Bilingual Document Alignment with Latent Semantic Indexing

We apply cross-lingual Latent Semantic Indexing to the Bilingual Document Alignment Task at WMT16. Reduced-rank singular value decomposition of a bilingual term-document matrix derived from known English/French page pairs in the training data allows us to map monolingual documents into a joint semantic space. Two variants of cosine similarity between the vectors that place each document into the joint semantic space are combined with a measure of string similarity between corresponding URLs to produce 1:1 alignments of English/French web pages in a variety of domains. The system achieves a recall of ca. 88% if no in-domain data is used for building the latent semantic model, and 93% if such data is included. Analysing the system's errors on the training data, we argue that evaluating aligner performance based on exact URL matches under-estimates their true performance and propose an alternative that is able to account for duplicates and near-duplicates in the underlying data.

==> tab-recall2.tex <==
\begin{table} 
\caption{Recall on the training set (in-domain target document pairs
  excluded from the bilingual term-document
  matrix.)}\label{tab-recall}\vspace{1em}

\renewcommand{\tabcolsep}{.4ex}
\begin{tabular*}{\linewidth}{%
cccc@{\extracolsep{\fill}}rrrrr@{$\,$}}
%% &
%% & \multicolumn{4}{c}{\textbf{recall (in \%)}}\\
%% \rotatebox{60}{cosine}%
%% &\rotatebox{60}{local cosine}%
%% &\rotatebox{60}{distance}%
%% &\rotatebox{60}{url similarity}
&&&&\multicolumn{5}{c}{\textbf{recall (in \%)}}\\
%\textbf{features} \\
\multicolumn{4}{c}{\textbf{features used}}
& strict\makebox[0pt][l]{\textsuperscript{a}} 
& 1.00\makebox[0pt][l]{\textsuperscript{b}}  
& 0.99\makebox[0pt][l]{\textsuperscript{b}} 
& 0.95\makebox[0pt][l]{\textsuperscript{b}} 
& 0.90\makebox[0pt][l]{\textsuperscript{b}} \\\hline
%\multicolumn{4}{r}{cos,lcos,dist,url}\\
%             strict   1.00   0.99   0.95   0.90
\multicolumn{4}{c}{cosine (cos)}
                      &   82.5 & 88.9 & 91.3 & 92.9 & 93.7\\
\multicolumn{4}{c}{``local'' cos. (lcos)}
                      &   83.3 & 88.9 & 91.4 & 92.8 & 93.6\\
\multicolumn{4}{c}{distance (dist)}
                      &   \\
\multicolumn{4}{c}{URL similarity (url)}
                      &   83.6 & 87.8 & 88.1 & 88.2 & 88.2\\
cos,&lcos&&           &   83.3 & 89.7 & 92.1 & 93.6 & 94.4\\
cos,&&dist&           &   \\
cos,&&&url            &   86.3 & 90.6 & 91.4 & 92.7 & 93.5\\
&lcos,&dist&          &   \\
&lcos,&&url           &   86.8 & 91.3 & 92.2 & 93.4 & 94.2\\
&&dist,&url           &   \\
cos,&lcos,&dist&      &   \\
cos,&lcos,&&url       &   88.0 & 92.5 & 93.4 & 94.7 & 95.5\\
&lcos,&dist,&uorl      &   \\
cos,&lcos,&dist,&url  &   \\\hline
\end{tabular*}

\begin{tabular*}{\linewidth}{ll}
\textsuperscript{a}& string match with the reference ULR pairs\\
\textsuperscript{b}& soft match based on document similarity with\\
& different similarity thresholds.
\end{tabular*}

\end{table}

